Quantum Machine Learning in Climate Change and Sustainability: a Review

Climate change and its impact on global sustainability are critical challenges, demanding innovative solutions that combine cutting-edge technologies and scientific insights. Quantum machine learning (QML) has emerged as a promising paradigm that harnesses the power of quantum computing to address complex problems in various domains including climate change and sustainability. In this work, we survey existing literature that applies quantum machine learning to solve climate change and sustainability-related problems. We review promising QML methodologies that have the potential to accelerate decarbonization including energy systems, climate data forecasting, climate monitoring, and hazardous events predictions. We discuss the challenges and current limitations of quantum machine learning approaches and provide an overview of potential opportunities and future work to leverage QML-based methods in the important area of climate change research.

==> literature_review.tex <==
QML 
Literature Review: Quantum Machine Learning and its applications
On the Capabilities of Quantum Machine Learning
Quantum technologies for climate change: Preliminary assessment







Energy Systems: 
On the Use of Quantum Reinforcement Learning in Energy-Efficiency Scenarios 
A Multiagent Quantum Deep Reinforcement  Learning Method for Distributed Frequency Control of Islanded Microgrids 
Quantum Technology & Quantum Neural Networks in Smart Grids Control: Premier Perspectives 
Quantum Neural Networks (QNN) Application in Weather Prediction of Smart Grids
Prediction of Solar Irradiance One Hour Ahead Based on Quantum Long Short-Term Memory Network 
Quantum computing and quantum artificial intelligence for renewable and sustainable energy: A emerging prospect towards climate neutrality
Distributed quantum multiagent deep meta reinforcement learning for area autonomy energy management of a multiarea microgrid
Application of Big Data and Machine Learning in Smart Grid, and Associated Security Concerns: A Review
A quantum-based approach for offensive security against cyber attacks in electrical infrastructure
Quantum Machine Learning for Photovoltaic Topology Optimization


Transportation
Blockchain Based Optimized Energy Trading for
E-Mobility Using Quantum Reinforcement Learning
Hybrid approach based combined allocation of electric vehicle charging stations and capacitors in distribution systems




Agriculture
A Comparative Study of Quantum and Classical Deep Learning for Intelligent Agriculture


Data Forecasting
ONE-STEP TIME SERIES FORECASTING USING VARIATIONAL QUANTUM CIRCUITS
Time Series Forecasting with Quantum Machine Learning Architectures 

Load Forecasting
Short-Term Load Forecasting Model Based on Quantum Elman Neural Networks
Short-Term Load Forecasting Model Based on the Fusion of PSRT and QCNN
Day-Ahead Spatiotemporal Wind Speed Forecasting 
Based on a Hybrid Model of Quantum and Residual 
Long Short-Term Memory Optimized by Particle 
Swarm Algorithm
Short-Term Multiple Load Forecasting Model of Regional Integrated Energy System Based on QWGRU-MTL


Weather forecasting
A Study on Quantum Machine Learning for Accurate and Efficient Weather Prediction 
Quantum Neural Networks (QNN) Application in Weather Prediction of Smart Grids
Prediction of Solar Irradiance One Hour Ahead Based on Quantum Long Short-Term Memory Network
Prediction of Solar Irradiation Using Quantum Support Vector Machine Learning Algorithm
THE EFFECT OF SUPERPOSITION AND ENTANGLEMENT ON HYBRID QUANTUM MACHINE LEARNING FOR WEATHER FORECASTING
Can a Quantum Computer be Applied for Numerical Weather Prediction? 
Hybrid Classical-Quantum Neural Network for Improving Space Weather Detection and Early Warning Alerts








RE forecasting
Prediction of Solar Irradiance One Hour Ahead Based on Quantum Long Short-Term Memory Network


Carbon Price Forecasting
Linear-layer-enhanced quantum long short-term memory for carbon price forecasting



Climate Monitoring
Satellite image classification using quantum machine learning
On Circuit-based Hybrid Quantum Neural Networks for Remote Sensing Imagery Classification
Quantum machine learning for image classification
Potential of Quantum Machine Learning for Processing Multispectral Earth Observation Data
MULTI-SPECTRAL IMAGE CLASSIFICATION WITH QUANTUM NEURAL NETWORK
Potential of Quantum Machine Learning for Processing Multispectral Earth Observation Data
Hybrid Classical-Quantum Neural Network for Improving Space Weather Detection and Early Warning Alerts
Quantum Artificial Intelligence for the Science of Climate Change








Climate Hazards Prediction
Classification of Potentially Hazardous Asteroids Using Supervised Quantum Machine Learning
Exploring Quantum Machine Learning (QML) for Earthquake Prediction
Analysis of Quantum Machine Learning Algorithms in Noisy Channels for Classification Tasks in the IoT Extreme Environment
Hybrid Classical-Quantum Neural Network for Improving Space Weather Detection and Early Warning Alerts










